Change a Bit to save Bytes: Compression for Floating Point Time-Series Data

The number of IoT devices is expected to continue its dramatic growth in the coming years and, with it, a growth in the amount of data to be transmitted, processed and stored. Compression techniques that support analytics directly on the compressed data could pave the way for systems to scale efficiently to these growing demands. This paper proposes two novel methods for preprocessing a stream of floating point data to improve the compression capabilities of various IoT data compressors. In particular, these techniques are shown to be helpful with recent compressors that allow for random access and analytics while maintaining good compression. Our techniques improve compression with reductions up to 80% when allowing for at most 1% of recovery error.

==> figures/nomenclature_table.tex <==
\begin{tabular}{clcl}
	\toprule
	\textbf{Notation} & \textbf{Meaning}               \\ \midrule
	DS & Dataset \\
	CR       & Compression Ratio       \\
	FP		&Floating Point \\
	$E_U$	&Unbiased Exponent, namely $E - 127$ \\
	$E_U^A$	& Unbiased exponent of the addendum A \\
	$E_U^{n_2}$	& Unbiased exponent of $n_2$ \\
	@ & Any bit value\\
	 \bottomrule
\end{tabular}


==> sections/Nomenclature.tex <==
\section{Nomenclature}
\label{sec:nomenclature}

\begin{table}[!t]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Nomenclature}
	\setlength\tabcolsep{5pt}
	\input{figures/nomenclature_table.tex}
	\label{tab:nomenclature}
\end{table}



See \autoref{tab:nomenclature} for a summary of our nomenclature.

